Koios: A Deep Learning Benchmark Suite for FPGA Architecture and CAD Research

With the prevalence of deep learning (DL) in many applications, researchers are investigating different ways of optimizing FPGA architecture and CAD to achieve better quality-of-results (QoR) on DL-based workloads. In this optimization process, benchmark circuits are an essential component; the QoR achieved on a set of benchmarks is the main driver for architecture and CAD design choices. However, current academic benchmark suites are inadequate, as they do not capture any designs from the DL domain. This work presents a new suite of DL acceleration benchmark circuits for FPGA architecture and CAD research, called Koios. This suite of 19 circuits covers a wide variety of accelerated neural networks, design sizes, implementation styles, abstraction levels, and numerical precisions. These designs are larger, more data parallel, more heterogeneous, more deeply pipelined, and utilize more FPGA architectural features compared to existing open-source benchmarks. This enables researchers to pin-point architectural inefficiencies for this class of workloads and optimize CAD tools on more realistic benchmarks that stress the CAD algorithms in different ways. In this paper, we describe the designs in our benchmark suite, present results of running them through the Verilog-to-Routing (VTR) flow using a recent FPGA architecture model, and identify key insights from the resulting metrics. On average, our benchmarks have 3.7x more netlist primitives, 1.8x and 4.7x higher DSP and BRAM densities, and 1.7x higher frequency with 1.9x more near-critical paths compared to the widely-used VTR suite. Finally, we present two example case studies showing how architectural exploration for DL-optimized FPGAs can be performed using our new benchmark suite.

==> benchmarks/attention.tex <==
\subsection{Attention layer} \label{attention}  

==> benchmarks/clstm.tex <==
\subsection{C-LSTM-like overlay} \label{c_lstm}  

==> benchmarks/conv_handcoded.tex <==
\subsection{Convolution layer} \label{conv_handcoded}  

==> benchmarks/conv_hls.tex <==
\subsection{Convolution layer (HLS)} \label{conv_hls}  

==> benchmarks/dla.tex <==
\subsection{Intel DLA-like Overlay} \label{intel_dla}  

==> benchmarks/eltwise.tex <==
\subsection{Elementwise layer} \label{eltwise}  

==> benchmarks/gemm.tex <==
\subsection{GEMM layer} \label{gemm}  

==> benchmarks/lstm.tex <==
\subsection{LSTM layer} \label{lstm}  

==> benchmarks/mlp_hls.tex <==
\subsection{MLP network - HLS} \label{leflow_mlp}  

==> benchmarks/reduction.tex <==
\subsection{Reduction layer} \label{reduction}  

==> benchmarks/rl.tex <==
\subsection{Reinforcement Learning accelerator} \label{rl_robot}  

==> benchmarks/softmax.tex <==
\subsection{Softmax layer} \label{softmax}  

==> benchmarks/spmv.tex <==
\subsection{SpMV layer} \label{spmv}  

==> benchmarks/tiny_darknet_hls.tex <==
\subsection{Tiny Darknet network - HLS} \label{tiny_darknet}  

==> benchmarks/tpu_v1.tex <==
\subsection{TPU-v1-like Overlay} \label{tpu_v1}  

==> benchmarks/tpu_v2.tex <==
\subsection{TPU-v2-like Overlay} \label{tpu_v2}  
